Nerflets: Local Radiance Fields for Efficient Structure-Aware 3D Scene Representation from 2D Supervision

We address efficient and structure-aware 3D scene representation from images. Nerflets are our key contribution -- a set of local neural radiance fields that together represent a scene. Each nerflet maintains its own spatial position, orientation, and extent, within which it contributes to panoptic, density, and radiance reconstructions. By leveraging only photometric and inferred panoptic image supervision, we can directly and jointly optimize the parameters of a set of nerflets so as to form a decomposed representation of the scene, where each object instance is represented by a group of nerflets. During experiments with indoor and outdoor environments, we find that nerflets: (1) fit and approximate the scene more efficiently than traditional global NeRFs, (2) allow the extraction of panoptic and photometric renderings from arbitrary views, and (3) enable tasks rare for NeRFs, such as 3D panoptic segmentation and interactive editing.

==> [CVPR 2023] nerflets/definitions.tex <==
\newcommand{\bfr}{\mathbf{r}}
\newcommand{\bfx}{\mathbf{x}}
\newcommand{\bfo}{\mathbf{o}}
\newcommand{\bfd}{\mathbf{d}}
\newcommand{\bfc}{\mathbf{c}}
\newcommand{\bfw}{\mathbf{w}}
\newcommand{\bfs}{\mathbf{s}}
\newcommand{\bfmu}{\boldsymbol{\mu}}

% \newcommand{\bfp}{\mathbf{p}}


\newcommand{\calL}{\mathcal{L}}


% Spacing commands
\setlength{\floatsep}{0.50\floatsep}
\setlength{\textfloatsep}{0.50\textfloatsep}
\setlength{\dblfloatsep}{0.50\dblfloatsep}
\setlength{\dbltextfloatsep}{0.50\dbltextfloatsep}
\setlength{\abovedisplayskip}{3pt}
\setlength{\belowdisplayskip}{3pt}


==> [CVPR 2023] nerflets/figures/blend.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=0.85\linewidth]{figures/blendf.pdf}
  \vspace{-0.7em}
   \caption{Sample and blend method illustration. Results from individual nerflets are mixed based on the influence values $g_i$ determined by the distance-based weighting function. The mixing is smooth but most locations in space are dominated by a single nerflet, even when there is some overlap.}
   \label{fig:blend}
\end{figure}

==> [CVPR 2023] nerflets/figures/kitti360_editing.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=1.0\linewidth]{figures/kitti360_edit.pdf}
  \vspace{-1.8em}
   \caption{KITTI-360 scene editing. We replace cars (top) or removing a sign instance (bottom).}
   \label{fig:kitti360_editing}
\end{figure}\textbf{}

==> [CVPR 2023] nerflets/figures/kitti360_panoptic.tex <==
\begin{figure*}[t]
  \centering
  \vspace{-0.5em}
  \includegraphics[width=\linewidth]{figures/kitti360_pan.pdf}
  \vspace{-2.0em}
   \caption{Visualization of nerflet outputs, trained on KITTI-360 images.}
   \label{fig:kitti360_panoptic}
\end{figure*}

==> [CVPR 2023] nerflets/figures/kitti360_photo.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{figures/kitti360_photof.pdf}
   \vspace{-1.8em}
   \caption{Novel view synthesis qualitative comparison. Nerflets outperform NeRF, Mip-NeRF, and FVS, and perform comparably to PNF with better performance in difficult areas (far left), possibly due to explicit spatial allocation of parameters.}
   \label{fig:kitti360_photo}
\end{figure}

==> [CVPR 2023] nerflets/figures/kitti360_semantic.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{figures/kitti360_sem.pdf}
     \vspace{-1.8em}
   \caption{Novel view semantic synthesis qualitative comparison. Nerflets outperform other methods, particularly with respect to details and thin structures.}
   \label{fig:kitti360_semantic}
\end{figure}

==> [CVPR 2023] nerflets/figures/nerflet_info.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=1.0\linewidth]{figures/diagram.pdf}
   \caption{Information maintained by a nerflet and NeRF. Compared to NeRF, a nerflet focuses only on a small portion of the scene determined by its influence function $g$ (Eq.~\ref{eq:influence_fun}), and thus it uses a miniature MLP to fit density $\sigma$ and color $\bfc$. Each nerflet also maintains a single semantic logit vector $\bfs_i$ and an assigned instance ID $\text{Ins}_i$. Together these parameters comprise a compact building block for our scene representation.}
   \label{fig:nerflet_info}
\end{figure}

==> [CVPR 2023] nerflets/figures/scannet_3d.tex <==
\begin{figure}[t]
  \centering
  \vspace{-0.3em}
  \includegraphics[width=\linewidth]{figures/scannet_3df.png}
  \vspace{-2.0em}
   \caption{A 3D mesh extracted from a ScanNet RGB sequence with nerflets, colorized according to predicted panoptic labels. Ground truth RGBD mesh with human-annotated labels is shown on the left. Nerflets successfully reconstruct and label a chair instance missing from the ground truth mesh.}
   \label{fig:scannet_3d}
\end{figure}

==> [CVPR 2023] nerflets/figures/scannet_editing.tex <==
\begin{figure}[t]
  \centering
    \vspace{-0.4em}
  \includegraphics[width=1.0\linewidth]{figures/scannet_edit.pdf}
  \vspace{-1.8em}
   \caption{Scene editing comparison with ObjectNeRF on a pair of ScanNet images shown in the ObjectNeRF paper. Notice the improved handling of free space during removal and the more accurate texture during duplication, both attributable to the simple ``copy-and-paste'' nature of nerflets manipulation. }
   \label{fig:scannet_editing}
\end{figure}

==> [CVPR 2023] nerflets/figures/scannet_nvs.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{figures/scannet_nvsf.pdf}
  \vspace{-1.8em}
   \caption{ScanNet qualitative result and comparison to DM-NeRF~\cite{wang2022dmnerf}. The comparison is on a ScanNet view synthesis example taken from the DM-NeRF paper.  Our results improve in terms of both image and segmentation quality- notice the better image rendering for the glass table, and the better segmentation of the chair legs, which even exceeds the ground truth quality.}
   \label{fig:scannet_nvs}
\end{figure}

==> [CVPR 2023] nerflets/figures/teaser.tex <==
\begin{strip}
  \centering
  \vspace{-4.3em}
%   \includegraphics[width=\textwidth]{figures/teaser_rtx.png}
  \includegraphics[width=\textwidth]{figures/teaser-v2.png}
  \vspace{-1.8em}
  \captionof{figure}{We propose to represent the scene with a set of local neural radiance fields, named nerflets, which are trained with only 2D supervision. Our representation is not only useful for 2D tasks such as novel view synthesis and panoptic segmentation, but also capable of solving 3D-oriented tasks such as 3D segmentation and scene editing. The key idea is our learned structured decomposition (top right).}
  \vspace{-0.4em}
  \label{fig:teaser}
\end{strip}

==> [CVPR 2023] nerflets/sections/abs.tex <==
% In this paper, we study the problem of 3D scene understanding and editing from only 2D supervision. We model the scene with a set of local neural radiance fields named nerflets. Each nerflet maintains its own position, orientation, extent, as well as density and radiance reconstruction. By leveraging only 2D photometric, semantic and instance supervision, we can directly optimize these nerflet parameters to form a decomposition of the scene, where each object instance is represented by a subset of nerflets. We show that by decomposing a scene into nerflets, we can not only fit and render from the scene more efficiently, but also generate an information-rich instance-level 3D representation, on which we can achieve not only high-quality image and segmentation renderings, but also 3D-oriented tasks such as scene editing, multi-view depth prediction, and 3D segmentation.

We address efficient and structure-aware 3D scene representation from images. \emph{Nerflets} are our key contribution-- a set of local neural radiance fields that together represent a scene. Each nerflet maintains its own spatial position, orientation, and extent, within which it contributes to panoptic, density, and radiance reconstructions. By leveraging only photometric and inferred panoptic image supervision, we can directly and jointly optimize the parameters of a set of nerflets so as to form a decomposed representation of the scene, where each object instance is represented by a group of nerflets.   During experiments with indoor and outdoor environments, we find that nerflets: (1) fit and approximate the scene more efficiently than traditional global NeRFs, (2) allow the extraction of panoptic and photometric renderings from arbitrary views, and (3) enable tasks rare for NeRFs, such as 3D panoptic segmentation and interactive editing. \href{https://jetd1.github.io/nerflets-web/}{Our project page}.


==> [CVPR 2023] nerflets/sections/background.tex <==

\reviseme{Let's try to squeeze this into method, or maybe assume it's already known?}
\textbf{Neural Radiance Field (NeRF)} Only recently, NeRF~\cite{mildenhall2021nerf} has been proposed to achieve photo-realistic novel view synthesis from only posed 2D images. Follow-up methods extend the framework in terms of generalizability~\cite{}, scalability~\cite{}, efficiency~\cite{}, interprebility~\cite{} and more information~\cite{}. Given a set of posed images $I_1$,...,$I_l$ of a scene with their known camera parameters $\Phi_1$,...,$\Phi_l$. NeRF~\cite{mildenhall2021nerf} uses an MLP to learn the 3D geometry and appearance information of the scene. More specifically, it learns a continuous scene function $F$ whose input is a location $\bfx=(x,y,z)$ and a viewing direction $\bfd = (\theta, \phi)$, and whose output is an emitted color $\bfc=(r,g,b)$ and volume density $\sigma$, representing local geometry and appearance information respectively. NeRF then use a discretized version of classical volume rendering~\cite{} to generate the estimated pixel color $\hat{C}(\bfr)$ for camera ray $\bfr(t)=\bfo+t\bfd$:
\begin{align}
\label{eq:nerf_raymarching}
\hat{C}(\bfr) &=\sum_{i=1}^N T_i \alpha_i \bfc_i, \\
\text{where\ \ }
 \alpha_i &= 1-\exp \left(-\sigma_i \delta_i\right), \\
%& T_i=\exp \left(-\sum_{j=1}^{i-1} \sigma_j \delta_j\right),
 T_i &=\prod_{j=1}^{i-1} (1-\alpha_j),
\end{align}
where $t_i$ are stratified samples along the ray in $N$ evenly-spaced bins, and $\delta_i=t_{i+1}-t_i$ the distance between adjacent samples.
% \xiaoshuai{I want to cover these equations for later reference. Separating this yields a very short preliminaries section.}


==> [CVPR 2023] nerflets/sections/conclusion.tex <==
\vspace{-0.5em}
In this work, we present nerflets, a novel 3D scene representation which decomposes the scene into a set of local neural fields. Past work demonstrated structure is useful for parsimony in MLP-based shape representation~\cite{genova2020local}, and we have found similar evidence extending that to scenes in this paper.
Thanks to the locality of each nerflet, our model is compact, efficient, and multi-view-consistent. Results of experiments on two challenging real-world datasets KITTI-360 and ScanNet demonstrate state-of-the-art performance for panoptic novel view synthesis, as well as competitive novel view synthesis and support for downstream tasks such as scene editing and 3D segmentation. 

Despite these positives, nerflets have several limitations. For example, we do not model dynamic content. Even though the representation is well-suited for handling rigid motions (as demonstrated in scene editing), that feature has not been investigated. Also, while individual nerflet radiance fields are capable of handling participating media, the overall representation may struggle to fit scenes where those effects cross semantic boundaries (e.g., foggy outdoor sequences). Finally, we currently assume a fixed number of nerflets for each scene, regardless of the scene complexity. However, it may be advantageous to prune, add, or otherwise dynamically adjust the number based on where they are needed (\eg where the loss is highest).  
Investigating these novel features is interesting for future work.

\pagebreak
\noindent\textbf{Acknowledgements.} We sincerely thank Yueyu Hu, Nilesh Kulkarni, Songyou Peng, Mikaela Angelina Uy, Boxin Wang, and Guandao Yang for useful discussion and help on experiments. We also thank Avneesh Sud for feedback on the manuscript.

==> [CVPR 2023] nerflets/sections/discussion.tex <==
% \input{tables/abl_semvsapp}



% \subsection{Scene Decomposition Quality}
\noindent\textbf{Scene Decomposition Quality:}
% \kyle{I added a text reference here to a figure I think we need- a visualization of the nerflets in 3D (could be just like the teaser, for more images). i.e., ``Does nerflet structure mirror the scene structure?''}.
Our insight was to create an irregular representation that mirrors the structure of the scene. Do nerflets succeed at achieving this scene decomposition? In Fig.~\ref{fig:kitti360_panoptic}, we show RGB and panoptic images alongside the underlying nerflet decomposition that generated them. We see that indeed, the nerflets do not cross object boundaries, do join together to represent large or complex objects, and do cover the scene content.

%\subsection{Robustness to Pseudo-Label Errors}

%\subsection{Decomposition}
%\reviseme{supp:Show decomposition results and individual nerflets renderings here.}

%\subsection{nerflets Distribution}
%We visualize the change of nerflets' spatial distribution during training. \xiaoshuai{write more}

% \subsection{Semantics Help Appearance}
\noindent\textbf{Semantics Help Appearance:}
\label{subsec:semvsapp}
One key insight about our approach is that the semantic structure of the nerflets decomposition is beneficial even for lower level tasks, like novel view synthesis. We perform an experiment on the KITTI-360 validation set and observe that when training without a semantic or instance loss (i.e., photometric and regularization losses only), nerflets achieve a PSNR of 20.95. But when adding the semantics loss, PSNR \textit{increases} to 22.43, because the nerflets end up more accurately positioned where the content of the scene is. This is also why we train with a higher semantic loss early in training, to encourage better nerflet positioning.


\input{tables/abl_reg}
% \subsection{Ablation Study}
\noindent\textbf{Ablation Study:}
\label{subsec:regularizers} 
Here we run a knock-out ablation study to validate the effectiveness of each of our regularization terms. Table~\ref{tab:abl_reg} shows that all regularization terms contribute to final performance quantitatively. $\calL_\text{density}$ is the most crucial term for learning a nice representation. It affects both image synthesis and segmentation performance, as it encourages nerflets to focus around actual scene content. $\calL_\text{radii}$, $\calL_{\ell_1}$ and $\calL_\mathrm{box}$ all also improve performance, due to their effect of forcing a more well-separated and active decomposition of the scene where all nerflets contribute to the final result.


% \subsection{Performance}
% \kyle{Let's move this somewhere else? Supplemental?}
\noindent\textbf{Performance:}
Nerflets have good performance due to their local structure. Our editor renders $320\times240$ top-$1$ editable volume images with 192 samples/pixel at 31 FPS with 4 A100 GPUs and 64 nerflets-- 457 million sample evaluations per second. %While this is not competitive with state of the art efficient rendering approaches that are focused only on RGB images, like Kilo-NeRF~\cite{reiser2021kilonerf}, we believe our approach is a good compromise that is both efficient and aligned with the scene structure, making it suitable for editing.

\vspace{-0.5em}

==> [CVPR 2023] nerflets/sections/exp.tex <==

In this section, we evaluate our method using 512 nerflets on multiple tasks with two challenging real-world datasets. Please see the supplemental for other hyperparameters.
%For outdoor experiments, we use the view synthesis scenes from KITTI-360~\cite{kitti360}. For indoor experiments, we use the subset of 8 scenes from ScanNet~\cite{dai2017scannet} used for tests in previous NeRF papers \cite{XXX}.

\noindent\textbf{KITTI-360:}
%We performed an extensive set of experiments to evaluate our model on multiple computer vision and graphics tasks, including novel view synthesis, 2D panoptic segmentation, scene editing and 3D segmentation. We perform experiments on both KITTI-360~\cite{kitti360}, which involves difficult forward facing cameras in complex outdoor scenes, and ScanNet~\cite{dai2017scannet}, which includes large-scale indoor scenes with a diverse set of objects.
For KITTI-360 experiments, we use the novel view synthesis split, and compare to Panoptic Neural Fields (PNF)~\cite{kundu2022panoptic}, a recent state of the art method for panoptic novel view synthesis (1st on the KITTI-360 leaderboard).  To generate 2D panoptic predictions for outdoor scenes, we use a Panoptic DeepLab~\cite{cheng2020panoptic} model trained on COCO~\cite{lin2014microsoft}.

\noindent\textbf{ScanNet:} For ScanNet experiments, we evaluate on 8 scenes as in DM-NeRF~\cite{wang2022dmnerf} and compare to recent baselines-- DM-NeRF~\cite{wang2022dmnerf}, which synthesizes both semantics and instance information, and Semantic-NeRF~\cite{Zhi21iccv_SemanticNeRF} which synthesizes semantics only.  To generate panoptic images for indoor scenes, we use PSPNet~\cite{zhao2017pyramid} and Mask R-CNN~\cite{he2017mask}. Please see the supplemental for important subtleties regarding how 2D supervision on ScanNet is achieved.


\input{tables/kitti360_leaderboard}
\input{figures/kitti360_photo}
\input{figures/kitti360_semantic}
\input{figures/scannet_nvs}

\input{figures/kitti360_editing}

\input{tables/scannet_nvs}
\input{figures/scannet_editing}
\input{figures/scannet_3d}
\input{tables/scannet3d_semins}
\input{figures/kitti360_panoptic}

\vspace{-1em}
\subsection{Results}
% \subsection{Novel View Synthesis}
\noindent\textbf{Novel View Synthesis:} 
We evaluate the performance of nerflets for novel view image synthesis on both KITTI-360 and ScanNet. As shown in Table~\ref{tab:kitti360}, on KITTI-360, our method achieves better PSNR than all other 2D supervised methods on the leaderboard and is competitive with PNF~\cite{kundu2022panoptic}, which utilizes 3D supervision. As shown in Figure~\ref{fig:kitti360_photo} our visual quality is approximately on par with PNF, and does particularly well in challenging areas. For complex indoor scenes in ScanNet (Table~\ref{tab:scannet}), we achieve the best performance for novel view synthesis under all settings (with or without instance supervision), including when compared to DM-NeRF~\cite{wang2022dmnerf}. In particular, nerflets achieve better object details (Figure~\ref{fig:scannet_nvs}), likely due to their explicit allocation of parameters to individual object instances. 

% \subsection{2D Panoptic Segmentation}
\noindent\textbf{2D Panoptic Segmentation:}
\label{sec:exp_panop2d}
Nerflets can render semantic and instance segmentations at novel views. We evaluate our 2D panoptic rendering performance quantitatively on both KITTI-360 (Table~\ref{tab:kitti360}) and ScanNet (Table~\ref{tab:scannet}). On both datasets, nerflets outperform all baselines in terms of semantic mIoU, even compared to the 3D-supervised PNF~\cite{kundu2022panoptic}. On the ScanNet dataset, we also show that nerflets outperform PSPNet~\cite{zhao2017pyramid} and Mask R-CNN~\cite{he2017mask} in terms of both mIoU and instance mAP, although those methods were used to generate the 2D supervision for our method. This is an indication that nerflets are not only expressive enough to represent the input masks despite their much lower-dimensional semantic parameterization, but also that nerflets are effectively fusing 2D information from multiple views into a better more consistent 3D whole. We further explore this in the supplemental material. Qualitatively, nerflets achieve better, more detailed segmentations compared to baseline methods (Figure~\ref{fig:kitti360_semantic}, Figure~\ref{fig:scannet_nvs}), particularly for thin structures.



% \subsection{Scene Editing}
\noindent\textbf{Scene Editing:}
\label{subsec:exp_editing}
In Figure~\ref{fig:kitti360_editing} and Figure~\ref{fig:scannet_editing}, we use the instance labels on nerflets to select individual objects, and then manipulate the nerflet structure directly to edit scenes. 
%object editing on KITTI-360 and ScanNet, respectively.
% With the semantic and instance labels in our representation, we can directly single out objects by their instance label, and perform scene editing tasks including inserting, removing, and transforming objects, by simply applying those operations to the nerflets with that instance label. 
No additional optimization is required, and editing can be done while rendering at interactive framerates (please see the video for a demonstration, the results here were rendered by the standard autodiff inference code for the paper).
%Fig.~\ref{fig:kitti360_editing} and Fig.~\ref{fig:scannet_editing} show several examples on KITTI-360 and ScanNet.
When compared to Object-NeRF on ScanNet (Figure~\ref{fig:scannet_editing}), nerflets generate cleaner results with more detail, thanks to their explicit structure and alignment with object boundaries. Using nerflets, empty scene regions will not carry any density after deletion, as there is nothing there to evaluate. In Figure~\ref{fig:kitti360_editing}, we demonstrate additional edits on KITTI-360, with similar results. These visualizations help to confirm that indeed, nerflets learn a precise and useful 3D decomposition of the scene.
%Also, we can achieve better visual quality because each object is represented by a different set of networks instead of a single MLP as in~\cite{yang2021objectnerf}. This alleviates the problem of network under-capacity.

% \subsection{3D Panoptic Reconstruction}
\noindent\textbf{3D Panoptic Reconstruction:}
In Figure~\ref{fig:scannet_3d}, we demonstrate the 3D capabilities of nerflets by extracting a panoptically labeled 3D mesh and comparing it to the ground truth. Surface extraction details are provided in the supplemental. We observe that the resulting mesh has both good reconstruction and panoptic quality compared to the ground truth. For example, nerflets even reveal a chair instance that is entirely absent in the ground truth mesh. We demonstrate this quantitatively by transferring nerflet representations to a set of ground truth 3D ScanNet meshes, comparing to existing 3D-labeling approaches in Table~\ref{tab:scannet3d}. We observe that nerflets outperform the similarly supervised multi-view fusion baseline, while adding instance capabilities. State of the art directly-3D supervised baselines are still more effective than nerflets when input geometry and a large 3D training corpus are available, but even so nerflets outperform some older 3D semantic and instance segmentation methods.

%\textbf{3D Panoptic Segmentation:}
% Since we can generate semantic and instance labels for arbitrary spatial location in the scene.
% In this this experiment, we evaluate the quality of our nerflet segmentations in 3D, by using them to label input point clouds with ground truth 3D labels. To do so, we simply query our representation in 3D at each input point location and transfer the semantic and instance labels. Quantitative results are shown in Table~\ref{tab:??} (A) . We observe that nerflets achieve reasonable 3D performance, trailing behind methods trained with large quantities of 3D supervision but outperforming similarly supervised methods for labeling 3D pointclouds from 2D, like multiview fusion, while also providing instance labels. A step beyond these methods, we can also extract a panoptically labeled 3D mesh from images using marching cubes (Figure~\ref{fig:scannet_3d}).

\vspace{-0.5em}

==> [CVPR 2023] nerflets/sections/intro.tex <==
% The ability to understand 3D scenes from 2D captures has been a long-standing challenge in computer vision. With the recent boom in augmented reality and autonomous driving, supporting this capability has become even more compelling, as it enables countless downstream tasks such as scene editing, navigation and robot manipulation.

% \xiaoshuai{starts more specifically here.}Over the past decade, we have seen a surge of research in this direction, and many related tasks such as scene classification~\cite{he2022masked,singh2022revisiting}, 2D object detection~\cite{redmon2016you,ren2015faster}, 2D semantic and instance segmentation~\cite{ronneberger2015u,he2017mask,liu2021swin} have been well-studied. This line of work, however, focuses on 2D reasoning of the scene with image-based feed-forward pipelines, while ignoring the underlying 3D structure of the scene. Also these pipelines only produce 2D information about the scene, which is error-prone and non-trivial for downstream tasks to utilize.

% On the other hand, with the recent progress on 3D backbones~\cite{qi2017pointnet,qi2017pointnet++,zhou2018voxelnet,graham2015sparse}, 3D-oriented tasks such as 3D detection and segmentation have seen great success~\cite{zhu2020ssn,cheng20212}. These pipelines could generate useful 3D information about the scene, but they are limited to explicit 3D inputs (\eg point clouds, or voxel grids) and thus require expensive 3D sensors. Moreover, most of these methods need explicit 3D supervision, which is extremely expensive to obtain compared to their 2D counterparts. 

% More recently, in parallel to these studies, neural 3D scene representations like NeRF~\cite{mildenhall2021nerf} have emerged as a powerful tool to represent 3D scene information such as density, and radiance in a unified manner with multi-layer perceptrons (MLPs). These representations are learned only from 2D images and are capable of capturing fine levels of geometry and texture detail for large-scale complex scenes~\cite{zhang2020nerf++,barron2021mip,zhang2022nerfusion}. However, most of the methods developed upon this technique focus on image reconstruction quality, with little attention paid to understanding scenes on an instance level. Among the few works that do consider scene understanding, some~\cite{} extend NeRF by adding an additional semantic MLP, predicting semantic logits along with density and radiance for ray marching. These works cannot extend to instance-level directly. Others~\cite{} utilize trained 3D detection or tracking models to generate additional information for the scene. However, these systems not only require 3D annotation for model pretraining, but also are prone to initial detection errors due to their reliance on pretrained models and multi-stage pipelines. For example, both PNF~\cite{} and NSG~\cite{} \reviseme{rely on accurate initial detection or tracking predictions. These models could fail on detection failures (\eg a missing object).}

%Why learn a compositional 3D representation from 2D supervision?  
% Outline:
% What we want (representation)
%   Define 3D output. Why 3D output? And, what do we want to do with this representation?
%   Define 2D supervision. Why 2D supervision?
%   What do we mean by efficient? What about end-to-end?
% What is currently out there?
%   Why doesn't it solve the problem?
% What is our solution?
%  What is unique about it?
%  What is good about it?
%  design an efficient end-to-end pipeline for learning a

% Semantics, instances, and appearance with a representation that is compact and efficient (parsimonious).

% What we want is this, and we want it for these tasks and useful for robotics applications, etc.
% What have other people done to produce such a method?
% Our solution is nerflets, describe them.
% These are the benefits nerflets, and why they are unique to nerflets.
% Key difference from current draft- attribute benefits to nerflets, they solve the problems and provide the benefits because of structure and ease of optimization, etc. Don't attribute to intro.
% TODO- in the future, write the whole intro in one sentence per paragraph first. Then extend only as needed.
% Move most of PNF comparison to related work.

This paper aims to produce a compact, efficient, and comprehensive 3D scene representation from only 2D images. Ideally, the representation should reconstruct appearances, infer semantics, and separate object instances, so that it can be used in a variety of computer vision and robotics tasks, including 2D and 3D panoptic segmentation, interactive scene editing, and novel view synthesis.


%The goal of this paper is to produce a structure-aware 3D scene representation from only 2D supervision. We will demonstrate the utility of such a structured representation by applying it to existing scene understanding tasks including 2D and 3D semantic and panoptic segmentation, interactive scene editing, and novel view synthesis.

%By ``structure-aware'', we mean a 3D representation composed of meaningful local building blocks. 
%Together, the building blocks describe the entire scene.
%They should be organized to correspond to useful high-level concepts-- objects and semantic classes. Individual elements should describe lower-level shape and texture information locally, for efficiency and generalization. 

% TODO(kgenova) The nerflets are of fixed complexity so they join together to create a single object. The fixed nerflet complexity enables efficient implementation, while objects are of variable complexity to multiple may join to make one instance. Where to mention this?

%By ``only 2D supervision,'' we mean that at both training time and inference time there are only images and image-based losses-- no ground truth 3D annotations of any kind, nor any input 3D points. While 3D \textit{outputs} are very useful, input images and image supervision are both more plentiful than 3D pointcloud scans or 3D ground truth labels~\cite{genova2021learning}.

Many previous approaches have attempted to generate rich 3D scene representations from images. PanopticFusion~\cite{narita2019panopticfusion} produces 3D panoptic labels from images, though it requires input depth measurements from specialized sensors. NeRF~\cite{mildenhall2021nerf} and its descendants~\cite{mueller2022instant, barron2021mip, barron2022mipnerf360, reiser2021kilonerf} produce 3D density and radiance fields that are useful for novel view synthesis, surface reconstruction, semantic segmentation~\cite{Zhi21iccv_SemanticNeRF, vora2021nesf}, and panoptic segmentation~\cite{kundu2022panoptic, wang2022dmnerf}. However, existing approaches require 3D ground truth supervision, are inefficient, or do not handle object instances.


% Our approach is to propose ``Nerflets,''


% Of course, we are not the first to tackle the 3D scene decomposition, image-based scene understanding, novel view synthesis, or some combination of the above.
% Many of these tasks are longstanding research goals in computer vision, with accompanying approaches (see Section~\ref{sec:rel}).
% Recently, NeRF~\cite{mildenhall2021nerf} and variants have been explored for novel view synthesis and understanding tasks, and we build upon this direction.
%Meanwhile, there are approaches for 3D panoptic segmentation~\cite{}, scene editing~\cite{}, and shape abstraction~\cite{}, all of which have various pros and cons, discussed in some detail in Section XX.

We propose \emph{nerflets}, a 3D scene representation with multiple local neural fields that are optimized jointly to describe the appearance, density, semantics, and object instances in a scene (Figure~\ref{fig:teaser}). Nerflets constitute a \textit{structured} and \textit{irregular} representation-- each is parameterized by a 3D center, a 3D XYZ rotation, and 3 (per-axis) radii in a 9-DOF coordinate frame.
The influence of every nerflet is modulated by a radial basis function (RBF) which falls off with increasing distance from the nerflet center according to its orientation and radii, ensuring that each nerflet contributes to a local part of the scene.  Within that region of influence, each nerflet has a miniature MLP to estimate density and radiance. It also stores one semantic logit vector describing the category (e.g., ``car'') of the nerflet, and one instance label indicating which real-world object it belongs to (e.g., ``the third car''). In Figure~\ref{fig:teaser}, each ellipsoid is a single nerflet, and they are colored according to their semantics.

A scene can contain any number of nerflets, they may be placed anywhere in space, and they may overlap, which provides the flexibility to model complex, sparse 3D scenes efficiently.  Since multiple nerflets can have the same instance label, they can combine to represent the density and radiance distributions of complex object instances.   Conversely, since each nerflet has only one instance label, the nerflets provide a complete decomposition of the scene into real-world objects. Nerflets therefore provide a 3D panoptic decomposition of a scene that can be rendered and edited.

Synthesizing images using nerflets proceeds with density-based volume rendering just as in NeRF~\cite{mildenhall2021nerf}.  However, instead of evaluating one large MLP at each point sample along a ray, we evaluate the small MLPs of only the nerflets near a sample. We average the results, weighting by the influence each nerflet has over that sample.  The rendering is fully-differentiable with respect to all continuous parameters of the nerflets. Fitting the nerflet representation is performed from a set of posed RGB images with a single training stage. After training, instance labels are assigned based on the scene structure, completing the representation.

\if 0

Notably, a nerflet does not have to describe everything nearby; the RBF is an ``upper-bound'' on its influence. Instead, each nerflet stores a variety of information about the local content of the scene. It has a single semantic logit vector, meaning it cannot span across multiple semantic classes-- though there may be multiple nerflets per semantic class in the scene.
Similarly, it has a single instance ID logit vector, so it cannot span multiple object instances-- although multiple nerflets may join together to describe a single complex instance containing more appearance information.
Finally, it has a miniature NeRF MLP describing density and color information, which describes either the whole or a part of the object that the nerflet belongs to.
The radial basis functions of multiple nerflets may overlap, but each learns to describe only the portion of the scene it is responsible for, allowing editing.
All the parameters of our representation are part of a single optimization with image-based losses.

Unique to our approach, the irregular 3D nerflet decomposition is optimized jointly with appearance and semantics, resulting in a learned 3D instance decomposition from only 2D supervision. As a result, we are able to create 3D instances for all classes with 2D panoptic supervision and even to separate and edit some 3D instances with only 2D semantic supervision. 

\fi

Experiments with indoor and outdoor datasets confirm the main benefits of nerflets.
We find that: 
1) Parsimony encourages the optimizer to decompose the scene into nerflets 
with consistent projections into novel panoptic images (Section~\ref{sec:exp_panop2d});
2) Semantic supervision can be beneficial to novel view synthesis (Section~\ref{subsec:semvsapp});
3) Structure encourages efficiency, compactness, and scalability (Section~\ref{sec:effient_evaluation}); and
4) the explicit decomposition of a scene improves human interpretability for easy interactive editing, including adding and removing objects (Section~\ref{subsec:exp_editing}).
These benefits enable state-of-the-art performance on the KITTI360~\cite{kitti360} novel semantic view synthesis benchmark, competitive performance on ScanNet 3D panoptic segmentation tasks with more limited supervision, and an interactive 3D editing tool that leverages the efficiency and 3D decomposition of nerflets.   

The following summarizes our main contributions:
\begin{itemize}[itemsep=0.1pt,topsep=2pt,leftmargin=2em]
    \item We propose a novel 3D scene representation made of small, posed, local neural fields named \emph{nerflets}.
    \item The pose, shape, panoptic, and appearance information of nerflets are all fit jointly in a single training stage, resulting in a comprehensive learned 3D decomposition from real RGB images of indoor or outdoor scenes.
    %\item Our scene decomposition is more compact, efficient, and explicit representation as compared to its global counterparts.
    \item 
    We test nerflets on 4 tasks- novel view synthesis, panoptic view synthesis, 3D panoptic segmentation and reconstruction, and interactive editing.
    %We demonstrate 3D instance-level decomposition and understanding of complex scenes with a neural field model from only 2D supervision, and apply it to 3D segmentation and interactive scene editing.%, while maintaining competitive photometric quality.
    \item We achieve 1st place on the KITTI-360 semantic novel view synthesis leaderboard.
    % \item We demonstrate the synergy between appearance and semantics synthesis-- adding a semantic synthesis task improves appearance performance. \reviseme{And vice-versa?}
    %\item Despite being trained on 2D losses, our compositional representation enables 3D tasks such as 3D segmentation and interactive scene editing.
\end{itemize}


%First, such a representation is a single approach that is useful for several popular vision tasks. Because of this, we are able to re-purpose supervision for one task to another task-- for example, performing 3D panoptic segmentation trained from a 2D panoptic image collection (Section XX).
% Parsimony is a useful prior-- by forcing an explicit and consistent ``car'' object to exist in 3D space and tying its appearance to its semantics, we are able to ensure better and more consistent projection of that instance into novel panoptic images (Section XX).
% Adding semantic supervision can be beneficial to appearance performance (Section XX).





% Unique to our approach, the irregular 3D nerflet decomposition is optimized jointly with appearance and semantics, resulting in a learned 3D instance decomposition from only 2D supervision. As a result, we are able to create 3D instances for all classes with 2D panoptic supervision, and even to separate and edit some 3D instances with only 2D semantic supervision. We demonstrate state of the art performance on the KITTI360 outdoor novel semantic view synthesis benchmark, competitive performance on ScanNet 3D panoptic segmentation tasks with more limited supervision, and an interactive 3D editing tool that leverages the efficiency and 3D decomposition of our representation.


% There are other benefits to nerflets. 
% %First, such a representation is a single approach that is useful for several popular vision tasks. Because of this, we are able to re-purpose supervision for one task to another task-- for example, performing 3D panoptic segmentation trained from a 2D panoptic image collection (Section XX).
% Parsimony is a useful prior-- by forcing an explicit and consistent ``car'' object to exist in 3D space and tying its appearance to its semantics, we are able to ensure better and more consistent projection of that instance into novel panoptic images (Section XX).
% Adding semantic supervision can be beneficial to appearance performance (Section XX).
% Structure encourages efficiency, compactness, and scalability-- multiple smaller independent networks can be executed dynamically only when the query is relevant to them (Section XX). 
% Finally, an explicit decomposition of a scene improves human interpretability for easy interactive editing, including translating, rotating, scaling, inserting, and removing objects (Section XX).



% is not fully end to end, and so prone to failure when the pretrained detector or tracker fails. 
% Why is this a desirable output representation, compared to training a 2D or 3D panoptic segmentation network directly? 
% First, a parsimonious output representation is 
% First, it is capable of synthesizing information from multiple 2D views and integrating them with 3D object priors-- we demonstrate these priors improve performance over off-the-shelf 2D panoptic segmentation networks.
% Intuitively, producing a ``car'' object in 3D space which realistically occludes like a car and is forced to have a single semantic class helps ensure car segmentations generalize to novel views. 
% Efficiency and compactness are also benefits- storing parameters locally on objects greatly improves memory locality, allowing multiple smaller independent networks that are each executed dynamically only when the query is relevant to them.
% Moving towards a full scene decomposition also improves human interpretability and makes interactive editing feasible, including translating, rotating, inserting, and removing objects.
%Similarly, requiring the ``sidewalk`` to be an instance of a sidewalk encourages 

% Why do we want this kind of representation? TODO: 1) Priors, 2) editing

% The representation should not only support high-quality novel view synthesis, but also record semantic and instance level information over the scene structure and support flexible scene manipulation such as object insertion, removal, rotation and translation.  
% To achieve these goals, we propose to represent scenes with components we call \textit{nerflets}. Each nerflet is a small local radiance field that has its pose (location and rotation) and extent. It also maintains a single semantic vector storing its semantic information. A nerflet MLP has a formulation similar to NeRF: it is a neural function mapping $(x,y,z)$ coordinates to density and radiance, $f_i(x,y,z,\theta,\phi)=(c,\sigma)$, but it describes this information locally rather than globally. During optimization, in addition to the MLP parameters, the poses and extents are also tuned so that nerflets cam migrate to cover the areas where objects exist. In this way, the learned scene-adapted model is more efficient due to not only smaller network sizes, but also because of the elimination of unnecessary samples. In addition, during optimization, we can utilize 2D semantic and instance segmentation maps from off-the-self 2D models and enforce nerflets to associate with only one object instance. By doing this, each instance in the scene, after optimization, is represented by a certain subset set of nerflets. This scene decomposition facilitates difficult 3D tasks, such as 3D scene segmentation, and enable scene editing. We present experiments on two real-world datasets -- KITTI-360~\cite{kitti360} and ScanNet~\cite{dai2017scannet} and compare our performance to competitive techniques for 2D and 3D scene understanding. \xiaoshuai{Do we need more method details here \eg rbf coverage, weighted sum.}


%\begin{itemize}
%    \item We are the first to achieve 3D instance-level understanding of complex scenes with a neural field model from only 2D supervision. \reviseme{We have shown state of the art performance on}
%    \item We propose a novel 3D scene representation composed of small posed local neural fields named \emph{nerflets}. Our model is end-to-end trained and optimized and is much more compact and efficient than previous object-aware neural representations. 
%    \item The decomposed representation facilitate down stream tasks such as scene editing and 3D segmentation.
%\end{itemize}

% We now describe our contributions relative to related work in more detail.

==> [CVPR 2023] nerflets/sections/limitations.tex <==
NOTE: THIS IS MOVED TO END OF CONCLUSION TO SAVE SPACE

Nerflets have several limitations. One limitation is that they do not model dynamic scene content. This is one potential direction for future work, because in principle the irregular nature of the representation could be leveraged to track moving or articulated objects.  Another is that we currently assume a fixed number of nerflets for the scene, regardless of the scene complexity, similar to a standard MLP. However, it may be advantageous to prune, add, or otherwise dynamically adjust the number based on where they are needed in the scene (e.g., where the loss is highest).

==> [CVPR 2023] nerflets/sections/method.tex <==
This section introduces our nerflet scene representation and our training and rendering method. As in NeRF~\cite{mildenhall2021nerf}, the input to our method is a set of posed 2D RGB images.
We first run an off-the-shelf 2D panoptic segmentation model~\cite{cheng2020panoptic} to generate predicted 2D semantic and instance images, which we use as a target during the optimization. 
Next, we optimize our core nerflet representation (Section~\ref{representation}) to convergence on photometric, semantic, instance, and regularization losses applied to images rendered with volumetric ray-marching~\cite{mildenhall2021nerf} (Section~\ref{sec:loss_functions}).
Finally, we assign instance labels to the nerflets based on the learned decomposition (Section~\ref{sec:instance_assignment}), at which point the representation is complete and ready for rendering or editing.

% (Section~\ref{}). 
% In Sec.~\ref{}, we describe our nerflets-based scene representation, which is composed of multiple posed nerflets and an optional background neural field. In Sec~\ref{}, we describe how to render from this compositional representation. In Sec~\ref{}, we explain further details on our loss functions and training schemes. In Sec~\ref{}, we explain the method we use to assign instance label with optimized scene representations. We cover details of our efficient implementation in Sec~\ref{}.

%\reviseme{overview, maybe summarize some key differences here with the pipeline figure?}

\subsection{Scene Representation}
\label{representation}

The core novelty of our framework is the nerflet scene representation. Nerflets are a structured representation, where the output radiance and panoptic fields are defined by blending the values produced by $N$ individual nerflets. 
%The scene is composed of a set of $N$ nerflets. 
%We begin by explaining a single nerflet, the building block of our approach.
%-- there is both an explicit structure (the number of nerflets, their locations, orientations, semantic and instance ids per nerflet), and the outputs they define-- a radiance and panoptic segmentation field for the scene which can be queried directly or rendered into novel views. We begin by describing the parameters stored on each nerflet.

% TODO small paragraph at some point about background in outdoor scene.
%Like NeRF, the radiance field maps a point position $\bfx \in \mathbb{R}^3$ and viewing direction $\bfd \in \mathbb{R}^2$ to output RGB + density values. 
%The panoptic field is defined over input positions $\bfx \in \mathbb{R}^3$, by combining the does not require evaluating any MLPs to compute; it is 

% Like vanilla NeRF, this representation takes a point position $\bfx \in \mathbb{R}^3$ and a viewing direction $\bfd \in \mathbb{R}^2$ as input. The outputs per query are color, and density.
% Additionally, there is also a semantic logit vector and an instance ID per nerflet, which can be access either 
% . The representation is composed of multiple local neural fields named \emph{nerflets}, and an optional background neural field for unbounded scene content (\eg distant buildings and sky) in large-scale scenes.


\noindent\textbf{Nerflet definition:} 
\input{figures/nerflet_info}
%Any content within the designated scene bound are represented by nerflets, 
Each nerflet stores local geometry, appearance, semantic, and instance information. As shown in Figure.~\ref{fig:nerflet_info}, a nerflet $i$ has 1) position and orientation parameters that define its influence function $g_i$ over space, 2) its own tiny MLP $f_i$ generating both density and radiance values, 3) a single semantic logit vector $\bfs_i$ storing its semantic information directly, and 4) an associated instance ID $\text{Ins}_i$. Compared to other semantics-aware NeRF methods~\cite{Zhi21iccv_SemanticNeRF, vora2021nesf}, we use a single logit vector to represent local semantic information instead of training an MLP to encode semantics. This aligns with our goal that a single nerflet should not span multiple classes or instances, and has the additional benefits of reducing the capacity burden of the MLP and providing a natural inductive bias towards 3D spatial consistency.
%This design reduces the capacity burden for the MLP and encourages meaningful spatial distribution of the nerflets when combined with the semantic supervision. \xiaoshuai{ablation study?}

\noindent\textbf{Pose and influence:}  Each nerflet has 9 pose parameters-- a 3D center $\bfmu_i$, 3 axis-aligned radii, and 3 rotation angles. We interpret these pose parameters in two ways. First, as a coordinate frame-- each nerflet can be rasterized directly for visualization by transforming an ellipsoid into the coordinate frame defined by the nerflet. This is useful for editing and understanding the scene structure (e.g., Figure~\ref{fig:teaser}).
The second way, more critical for rendering, is via an influence function $g_i(\bfx)$ defined by the same 9 pose parameters. $g_i$ is an analytic radial basis function (RBF) based on scaled anisotropic multivariate Gaussians~\cite{genova2019learning, genova2020local}
\begin{align}
\label{eq:influence_fun}
g_i(\bfx)=\eta\exp \left(-\frac{1}{2\tau}\left(\bfx-\bfmu_i\right)^T \Sigma_i^{-1}\left(\bfx-\bfmu_i\right)\right).
\end{align}
$\bfmu_i$ is the center of the basis function and $\Sigma_i$ is a 6-DOF covariance matrix. The covariance matrix is determined by 3 Euler-angle rotation angles and 3 axis-aligned radii that are the reciprocal of variance along each principal axis. These 9 parameters provide a fast and compact way to evaluate a region of influence for each nerflet without evaluating any neural network. This property is crucial for our fast training and evaluation, which will be introduced later.  $\eta$ is a scaling hyper-parameter set to 5 for all experiments, and $\tau$ is a scheduled temperature hyper-parameter used to control the falloff hardness. $\tau$ is reduced after each training epoch to minimize overlap between nerflets gradually.



% \subsection{Rendering with Nerflets}
\input{figures/blend}
\noindent\textbf{Rendering and blending:}
Given a scene represented by $N$ nerflets, we can render 2D images with volume rendering, as in NeRF:
\begin{align}
\label{eq:nerf_raymarching}
\hat{C}(\bfr) &=\sum_{k=1}^K T_k \alpha_k \bfc_k, \\
\text{where\ \ }
 \alpha_k &= 1-\exp \left(-\sigma_k \delta_k\right), \\
%& T_i=\exp \left(-\sum_{j=1}^{i-1} \sigma_j \delta_j\right),
\label{eq:nerf_transmission}
 T_k &=\prod_{j=1}^{k-1} (1-\alpha_j).
\end{align}
$\hat{C}(\bfr)$ is the final color of ray $\bfr$, $T_k$ is transmission at the $k$-th sample along the ray, $\alpha_k$ is the opacity of the sample, $\bfc_k$ is the color at the sample, $\delta_k$ is the thickness of the current sample on the ray, and $\sigma_k$ is the density at the sample. We denote $k$ for the index of the sample along a ray, $K$ total number of samples and reserve $i$ for the index of the nerflet.

The biggest difference from NeRF is that instead of employing a single large MLP to produce $\bfc_k$ and $\sigma_k$, we combine values produced by individual nerflets using their influence weights (Figure~\ref{fig:blend}).
We query individual nerflet MLPs $f_i$ at the $k$-th input sample $(\text{pos}, \text{dir})=(\bfx_k, \bfd)$ along the ray, producing producing $N$ values $\sigma_{k,i}$ and $\bfc_{k,i}$ for nerflets labeled $i \in [1,N]$.
We then map the individual nerflet $\sigma_{k,i}$ values to $\alpha_{k,i}$ for rendering using $\delta_k$ and Equation~\ref{eq:nerf_raymarching}.
Finally, we take a weighted average of the $N$ individual nerflet color and $\alpha$ values to produce $\bfc_k$ and $\alpha_k$:
\begin{align}
    \label{eq:nerflet_render_color}
    \bfc_k &= \sum_{i=1}^{N}\hat{g}_i(\bfx_k)\bfc_{k,i}, \\
    \label{eq:nerflet_render_alpha}
    \alpha_k &= \sum_{i=1}^{N}\hat{g}_i(\bfx_k)\alpha_{k,i}, \\
    \label{eq:nerflet_render_g_norm}
    \text{where\ \ } \hat{g}_i(\bfx_k) &= \frac{g_i(\bfx_k)}{\sum_{j=1}^N{g_j(\bfx_k)+\epsilon}}.
\end{align}
$\epsilon$ is a factor allowing smooth decay to zero in empty space, with $\Sigma g_i(\bfx_k) \sim \epsilon$. 
% Note we blend individual nerflet $\alpha$ values rather than $\sigma$ values, as we found this to perform better, possibly due to more consistent scale of opacity values. 
After blending, the $\alpha_k$ and $\bfc_k$ values are used directly for ray marching as in Eq.~\ref{eq:nerf_raymarching}-\ref{eq:nerf_transmission} to generate final pixel color values $\hat{C}(\bfr)$, as in NeRF.

While in principle we should evaluate all nerflet MLPs in the scene in this step, as gaussian RBFs have infinite support, we do not do this. Typically, $g_i$ is dominated by one or at most a handful of nerflets that are close to the sample.
%especially after convergence, as our losses introduced in Sec.~\ref{sec:loss_functions} discourage nerflets from overlapping. 
Therefore, we evaluate only the nearby MLPs, improving performance and scalability. This is implemented with our custom CUDA kernel, which will be introduced in Sec.~\ref{sec:effient_evaluation}. More distant nerflets are omitted from the average.

To generate semantic images, we average the per-nerflet semantic logit vector for each point sample in the same way described for color values $\bfc_{k,i}$ above.

To handle instances, we first compute a \emph{nerflet influence activation} function $\bfw \in \mathbb{R}^n$ for each point sample:
\begin{align}
    \label{eq:nerflet_influence_map}
%    \bfw = \sum_{i=0}^{n}\mathbb{1}_i\hat{g}_i(\bfx)
    \bfw(\bfx) = \text{SoftMax}([\sigma_1g_1(\bfx),\dots,\sigma_Ng_N(\bfx)]).
\end{align}
$\sigma_i$ is the density evaluation for $\bfx$ on the $i$-th nerflet. This value intuitively represents how much influence each nerflet has over a given point sample, and can be accumulated by ray marching to generate a nerflet influence map $W(\bfr)$ for each ray $\bfr$. $W(\bfr)$ continuously captures which nerflet is dominant for each final pixel value, and is used by our influence loss described in Section~\ref{sec:loss_functions}. To assign a discrete instance label to a query position or ray, we take $\mathrm{argmax}_{i \in [N]} w(\bfr)$ or $\mathrm{argmax}_{i \in [N]} W(r)$, respectively to get $i$, then output $\text{Ins}_i$, the instance of that nerflet.

% When working with unbounded outdoor scene, we follow~\cite{zhang2020nerf++} and draw $M$ point samples from the background neural field $f_\text{bg}$ in addition to $N$ nerflet-supported samples along the ray $\bfr$. These samples are accumulated together through ray marching to generate final color $\hat{C}(\bfr)$ and semantic logits $\hat{S}(\bfr)$.


\noindent\textbf{Unbounded scenes:} Nerflets support both indoor (bounded) and outdoor (unbounded) scenes. To handle unbounded scenes, we add a single MLP $f_\text{far}$ to evaluate samples outside a large scene bounding box. We draw $M$ additional samples for these points at the end of the ray, which we concatenate after our blended RGB$\alpha$ values and composite. We use the scheme proposed by Zhang \etal~\cite{zhang2020nerf++}, with an added semantics branch, though as the content is very distant and nearly directional, many other approaches would likely work well (e.g., an environment map).


\subsection{Loss Function}
\label{sec:loss_functions}
During training, we jointly optimize all network parameters as well as the pose of the nerflets. In this way, each nerflet can be pushed by gradients to ``move'' across the scene, and focus on a specific portion of it.  We expect a final decomposition mirroring the scene, with more nerflets on complex objects, and use multiple losses to that end.
%In this way, the parameters are dynamically allocated to regions of the scene with highest complexity.

The loss function is broken up into rgb, semantic, instance, and regularization terms:
\begin{align}
    \label{eq:losses}
    \calL = \calL_\text{rgb} + \calL_\text{sem} + \calL_\text{ins} + \calL_\text{reg}. 
\end{align}

$\mathbf{\calL_{rgb}}$\textbf{:} The RGB loss $\calL_\text{rgb}$ is the mean squared error between the synthesized color $\hat{C}$ and the ground truth color $C$ averaged over a batch of sampled rays, as in the original NeRF. The one change is that we weight this loss with a schedule parameter that is 0.0 at step 0. We gradually increase this value to 1.0 during training to prevent early overfitting to high frequency appearance information.

$\mathbf{\calL_{sem}}$\textbf{:} Our semantic loss $\calL_\text{sem}$ compares the volume-rendered semantic logits pixel with the Panoptic Deeplab prediction~\cite{cheng2020panoptic}. We use a per-pixel softmax-cross-entropy function for this loss.

$\mathbf{\calL_{ins}}$\textbf{:} The instance loss is defined as:
\begin{align}
    \label{eq:instance_loss}
    \calL_\text{ins} = -\frac{1}{P}\sum_{(\bfr_1, \bfr_2)} ||W(\bfr_1) - W(\bfr_2)||_1.
\end{align}
% \begin{align}
%     \label{eq:instance_loss}
%     \calL_\text{ins} = -\frac{1}{K}\sum_{\substack{I \in \text{Batch}, \bfr_1, \bfr_2 \in I, \\ \text{Ins}(\bfr_1) \neq \text{Ins}(\bfr_2)}} ||W(\bfr_1) - W(\bfr_2)||_1.
% \end{align}
That is, we sample $P$ ray pairs $(\bfr_1, \bfr_2)$ that are from the same class but different instances according to the instance segmentation model prediction, and enforce them to have different influence maps.
While this approach is somewhat indirect, well separated nerflets can be easily assigned instance labels (Section~\ref{sec:instance_assignment}), and it has the advantage of avoiding topology issues due to a variable number of instances in the scene while still achieving an analysis-by-synthesis loss targeting the instance decomposition. It is also compatible with the inconsistent instance ID labelings across different 2D panoptic image predictions.
Ray pairs $(\bfr_1,\bfr_2)$ are chosen within in an $L \times L$ pixel window per-batch for training efficiency.

$\mathbf{\calL_{reg}}$\textbf{:} 
Our regularization loss has several terms to make the structure of the nerflets better mirror the structure of the scene--
\begin{align}
    \label{eq:losses_reg}
    \calL_\text{reg} = \calL_\text{density} + \calL_\text{radii} + \calL_{\ell_1} + \calL_\text{box}. 
\end{align}
In addition to the intuitions described below, each of these is validated in a knock-out ablation study (Sec.~\ref{subsec:regularizers}) and tested on multiple datasets, to reduce the risk of overfitting to one setting.

First, to minimize unnecessary nerflet overlap within objects and reduce scene clutter, we penalize the $L_2$ norm of the radii of the nerflets ($\calL_{radii}$). To encourage sparsity where possible, we penalize the $L_1$ norm of the nerflet influence values at the sample locations ($\calL_{\ell_1}$). We also require nerflets to stay within their scene bounding box, penalizing:
\begin{align}
    \sum_{d \in \{x,y,z\}} \max(x_d - \mathrm{box}_{\mathrm{max}}, \mathrm{box}_{\mathrm{min}} - x_d, 0).
\end{align}
This reduces risk of ``dead'' nerflets, where a nerflet is far from the scene content, so it does not contribute to the loss, and therefore would receive no gradient.

Finally, we incorporate a ``density'' regularization loss $\calL_\text{density}$, which substantially improves the decomposition quality:
%$\mathbf{\calL_{density}}$\textbf{:} For editing and performance reasons (Section~\ref{}), it is beneficial to encourage nerflet centers to be positioned inside the object they describe. To achieve this, we apply the ``density'' loss , defined as:
\begin{align}
    \label{eq:density_loss}
    \calL_\text{density} = -\frac{1}{D}\sum_{i=1}^n\sum\nolimits_{\bfx\sim\mathcal{N}(\bfmu_i, \Sigma_i)}\sigma(\bfx).
\end{align}
$\mathcal{N}(\bfmu_i, \Sigma_i)$ represents the underlying multivariate gaussian distribution for the $i$-th nerflet and $D$ is the number of samples drawn. This term rewards a nerflet for creating density near its center location. As a result, nerflets end up centered inside the objects they reconstruct.


%temperature adjusting/weight filtering/top-k evaluation/mention coarse-to-fine/radii sum pen/cuda kernel 

%\subsection{Pseudo Novel View Label}

\subsection{Instance Label Assignment}
\label{sec:instance_assignment}
Given an optimized scene representation, we use a greedy merge algorithm to group the nerflets and associate them with actual object instances. We first pick an arbitrary 2D instance image, and render the associated nerflet influence map $W(\bfr)$ for the image. We then assign the nerflets most responsible for rendering each 2D instance to a 3D instance based on it. We proceed to the next image, assigning nerflets to new or existing 3D instances as needed. Because the nerflets have been optimized to project to only a single 2D instance in the training images, this stage is not prone to failure unless the 2D panoptic images disagree strongly. See the supplemental for additional details.



%\subsection{Maybe: 3D Scene Editing and Segmentation}
%\label{subsec:3dtasks}
%\xiaoshuai{Seem to be too straight-forward to cover in the paper.}

\subsection{Efficient Nerflet Evaluation}
\label{sec:effient_evaluation}
\noindent\textbf{Top-$k$ Evaluation:} Instead of evaluating all nerflet MLPs in a scene as in Eq.~\ref{eq:nerflet_render_color}-\ref{eq:nerflet_influence_map}, we use the $g_i$ influence values to filter out distant and irrelevant nerflets in two ways. First, we truncate all nerflet influences below some trivial threshold to 0-- there is no need to evaluate the MLP at all if it has limited support. In free space, often all MLPs can be ignored this way. Next, we implement a ``top-$k$'' MLP evaluation CUDA kernel that is compatible with the autodiff training and inference framework. This kernel evaluates only the highest influence nerflet MLPs associated with each sample. We use $k=16$ for both training and visualizations in this paper, although even more aggressive pruning is quite similar in image quality (e.g., a difference of only $\sim0.05$ PSNR between top-16 and top-3) and provides a substantial reduction in compute. A top-$k$ ablation study is available in the supplemental.

\noindent\textbf{Interactive Visualization and Scene Editing:}
We develop an interactive visualizer combining CUDA and OpenGL for nerflets that takes advantage of their structure, efficiency, rendering quality, and panoptic decomposition of the scene. Details are available in the supplemental. The key insight enabling efficient evaluation is that nerflets have a good sparsity pattern for acceleration -- they are sparse with consistent local structure. We greatly reduce computation with the following two pass approach. In the first pass, we determine where in the volumetric sample grid nerflets have high enough influence to contribute to the final image. In the second pass, we evaluate small spatially adjacent subgrids for a particular nerflet MLP, which is generally high-influence for all samples in the subgrid due to the low spatial frequency of the RBF function. This amortizes the memory bandwidth of loading the MLP layers into shared memory. This approach is not as fast as InstantNGP~\cite{mueller2022instant}, but is still interactive and has the advantage of mirroring the scene structure.



==> [CVPR 2023] nerflets/sections/rel.tex <==
Recently, the success of deep learning approaches for both computer vision and graphics tasks has enabled researchers to reconstruct and reason about 3D scenes under various settings. We review related work on segmentation and neural field based scene representations.

\vspace*{2mm}\noindent
\textbf{Semantic, Instance, and Panoptic Segmentation:} There are many methods designed for semantic, instance, and/or panoptic~\cite{kirillov2019panoptic} segmentation.
The most popular approaches are fully-supervised and operate within a single input data modality.
For example, 2D approaches~\cite{ronneberger2015u,long2015fully,badrinarayanan2017segnet,chen2017deeplab,zhao2017pyramid,zheng2021rethinking,he2017mask,liu2021swin,zhang2022resnest} are usually based on CNN or transformer backbones and associate each pixel in an image with certain semantic or instance labels. We leverage a trained 2D panoptic model, Panoptic Deeplab~\cite{cheng2020panoptic}, in our framework.

Similar frameworks have been proposed to solve 3D segmentation tasks for 3D point clouds \cite{pham2019jsis3d,qi2017pointnet,qi2017pointnet++,shi2019pv,thomas2019kpconv}, meshes \cite{hanocka2019meshcnn,huang2019texturenet}, voxel grids \cite{graham2015sparse,song2017semantic}, and octrees \cite{riegler2017octnet}.
%Compared to 2D approaches, 3D segmentation methods give more useful results for direct application in downstream tasks.
However, these methods typically require a large amount of annotated 3D data, which is expensive to obtain.

To avoid the need for 3D annotations, several multiview fusion approaches have explored aggregating 2D image semantic features onto a pointcloud or mesh using
weighted averaging \cite{hermans2014dense,kundu2020virtual,vineet2015incremental, armeni20193d}, conditional random fields (CRFs) \cite{kundu2014joint,mccormac2017semanticfusion}, and bayesian fusions \cite{ma2017multi,vineet2015incremental,zhang2019large}. There have also been approaches like 2D3DNet~\cite{genova2021learning} that combine both 2D mutiview fusion with a 3D model.

In contrast to these methods, ours builds a complete 3D representation including geometry, appearance, semantic, and instance information from only 2D inputs and without any input 3D substrate such as a mesh or a point cloud.

% To address the data scarcity problem, another line of work fuse information from 2D views to achieve 3D segmentation~\cite{,armeni20193d,kundu2020virtual,genova2021learning,mascaro2021diffuser}. For example, Kundu \etal~\cite{kundu2020virtual} propose to render a textured mesh into images and then extract semantic features from these images. The 2D features are then unprojected and fused onto the mesh to obtain a 3D segmentation. Genova \etal~\cite{genova2021learning} propose to train a 3D model from pseudo-labels derived from 2D segmentation maps using multi-view fusion.

% 
% 
% 
%

%Unsupervised methods and openset methods?

%\textbf{\reviseme{Explicit Scene Representations:}}

%\textbf{Implicit Representations:} Our approach draws inspiration from recent trend of implicit shape and scene representations. We have seen great success in using implict surface functions to represent shape~\cite{}. A line of work focuses on structured shape representations, which decomposes complex shapes into a set of fixed or deformed primitives~\cite{}. These methods are typically more scalable and efficient, and have improved the state of the art in shape reconstruction~\cite{} and completion tasks~\cite{}. \xiaoshuai{maybe separate this paragraph into a new subsection?}

%In parallel to these studies, neural radiance field (NeRF)~\cite{mildenhall2021nerf} has been proposed to achieve photo-realistic novel view synthesis from input posed 2D images. Follow-up methods extend the framework in terms of generalizability~\cite{}, scalability~\cite{}, efficiency~\cite{}, interprebility~\cite{} and more information~\cite{}. Among these methods, \reviseme{talk about kilo-nerf}. \reviseme{Talk about NSG and PNF}. 

% Make pipeline show on page 3, before method:
%\input{figures/pipeline}

\vspace*{2mm}\noindent
\textbf{Scene Understanding with NeRF:}
NeRF~\cite{mildenhall2021nerf} and subsequent work~\cite{kundu2022panoptic,ost2021neural,yang2021objectnerf,Zhi:etal:ICCV2021,vora2021nesf,kobayashi2022decomposing} show the promise of neural radiance fields for tasks beyond novel view synthesis, including 3D reconstruction, semantic segmentation, and panoptic segmentation.   
%Recent examples include PNF~\cite{kundu2022panoptic}, NSG~\cite{ost2021neural}, ObjectNeRF~\cite{yang2021objectnerf}, SemanticNeRF~\cite{Zhi:etal:ICCV2021}, NeSF~\cite{vora2021nesf}, and DFF~\cite{kobayashi2022decomposing}.
For example, SemanticNeRF~\cite{Zhi:etal:ICCV2021}, and NeSF~\cite{vora2021nesf} are useful for semantic understanding, but do not consider object instances.
DFF~\cite{kobayashi2022decomposing} leverages the power of large language models for semantic understanding, but similarly does not produce object instances.
ObjectNeRF~\cite{yang2021objectnerf} and NSG~\cite{ost2021neural} are useful for object editing, but do not produce a full panoptic decomposition or support efficient interactive editing.  None of these methods produce a complete scene representation in the way that nerflets do.

Panoptic Neural Fields (PNF)~\cite{kundu2022panoptic} is very relevant to our paper as it supports both semantic scene understanding and object-level scene editing.  PNF first runs a 3D object detector and then a tracker to create an input set of object tracks.   They then fit an individual MLP for each object track and another special ``stuff'' MLP for the remainder of the scene. 
This is a compelling and effective approach which supports moving objects, but it does not solve our target problem. It 1) requires expensive ground truth 3D supervision for the detector and tracker that are only available for some classes, and
%2) only produces a local representation for a limited number of ``thing'' classes like car, truck, and pedestrian, and 
2) has a fixed 3D scene decomposition that is provided by the input tracker results.
This last point means that it can fail when the detector or tracker fails, even if a multi-view analysis-by-synthesis appearance loss, like in NeRF, would have been able to force a correct prediction by requiring all pixels to be described by some object instance.
By comparison, nerflets require only 2D supervision, support any class for which 2D panoptic segmentations are available, and optimize most parameters jointly, improving efficiency and instance recall.

DM-NeRF~\cite{wang2022dmnerf} is highly related concurrent work. It learns an object decomposition of a scene, but does not provide the explicit structure, full panoptic decomposition, or easy interactive editing of nerflets. In particular, a large MLP decodes spatial positions to object identity vectors, and editing therefore requires careful consideration-- an inverse query algorithm~\cite{wang2022dmnerf}. By contrast, nerflets can be edited directly as geometric primitives. We compare quantitatively to both PNF and DM-NeRF in Section~\ref{sec:exp}.



\vspace*{2mm}\noindent
\textbf{Structured NeRF Representations:} 
One of the key advantages of nerflets is their irregular structure, which has been investigated in other contexts. Many existing approaches exploit structure for efficiency~\cite{mueller2022instant,reiser2021kilonerf,SunSC22,wu2021diver,lombardi2021mixture}, compactness~\cite{liu2020neural}, scalability~\cite{turki2022mega,zhang2022nerfusion}, human-interpretability~\cite{ost2021neural}, parsimony~\cite{genova2020local}, or editability\cite{kundu2022panoptic,yang2021objectnerf}.
%This includes several NeRF-based or inspired methods~\cite{reiser2021kilonerf, liu2020neural, wu2021diver, SunSC22, turki2022mega, mueller2022instant,yu_and_fridovichkeil2021plenoxels}.
For example, Kilo-NeRF~\cite{reiser2021kilonerf} and DiVER~\cite{wu2021diver} exploit regular grids of MLPs or features to improve the efficiency of NeRF novel view synthesis. MVP~\cite{lombardi2021mixture} builds an irregular primitive-based representation for real-time portrait rendering, but requires explicit scene geometry inputs to initialize the primitives and freezes their location after initialization. We take inspiration from these approaches, which achieve impressive performance through local structure, and apply their insights to panoptic segmentation and editing. Unlike these approaches, nerflets can conform to an object's extent and then move as it is edited.
In the future, more benefits of exploring irregular NeRF representations could include tracking a moving object or allowing for a consistent local coordinate frame for learning 3D priors.

%\tom{ Move this reference to methods section}
%SIF~\cite{genova2019learning} and LDIF~\cite{genova2020local} are relevant structured shape representations. We base our radial basis functions on this approach, although we only use the basis functions to interpolate MLPs, rather than directly representing shapes as their level set. \reviseme{think about more related work in this area we should cite.} 



==> [CVPR 2023] nerflets/tables/abl_reg.tex <==
\begin{table}
\centering
% \resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
\vspace{-0.6em}
\begin{tabular}{lccc}
\hline
                               & PSNR             & mIOU              &mAP\footnotesize{0.5}\\ \hline
w/o $\calL_\text{density}$     & 20.85            & 63.31             & 11.20  \\
w/o $\calL_\text{radii}$       & 27.23            & 72.43             & 26.32  \\ 
w/o $\calL_{\ell_1}$           & 28.83            & 68.23             & 21.74  \\
w/o $\calL_\mathrm{box}$       & 28.93            & 72.14             & 29.88  \\  
full model                     & \textbf{29.12}   & \textbf{73.63}    & \textbf{31.32}  \\

\hline
\end{tabular}
%} %< \resizebox
\vspace{-0.8em}
\caption{
Ablation experiment on ScanNet for the effectiveness of our regularization terms-- density loss $\calL_\text{density}$, radii penalty $\calL_\text{radii}$, influence sparsity loss $\calL_{\ell_1}$ and scene box loss. $\calL_\mathrm{box}$
} % \caption
\label{tab:abl_reg}
\end{table}

==> [CVPR 2023] nerflets/tables/abl_semvsapp.tex <==
\begin{table}
\centering
\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
\begin{tabular}{lccc}
\hline
                             & PSNR             & SSIM              & LPIPS  \\ \hline
Ours (w/o sem supervision)   & 20.95            & 0.778             & 0.343  \\
Ours (full model)            & \textbf{22.43}   & \textbf{0.820}    & \textbf{0.212}  \\  \hline
\end{tabular}
} %< \resizebox
\caption{
% 
Ablation experiment on our KITTI-360 validation set for the effectiveness of our semantic supervision. Representation learned with semantic supervision also achieves better performance on novel view synthesis.
} % \caption
\label{tab:abl_semvsapp}
\end{table}

==> [CVPR 2023] nerflets/tables/kitti360_leaderboard.tex <==
\begin{table}
\centering
\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
\begin{tabular}{lccc}
\hline
\multicolumn{1}{p{2cm}}{Method}                                                           & \multicolumn{1}{p{2cm}}{\centering Appearance \\ PSNR}  & \multicolumn{1}{p{2cm}}{\centering Semantics \\ mIOU} & \multicolumn{1}{p{2cm}}{\centering Worst Case \\ kFLOPs} \\ \hline
PBNR~\cite{kopanas2021point} + PSPNet~\cite{zhao2017pyramid}     & 19.91  & 65.07  &  - \\
FVS~\cite{Riegler2020ECCV} +  PSPNet~\cite{zhao2017pyramid}      & 20.00  & 67.08  &  - \\
NeRF~\cite{mildenhall2021nerf} + PSPNet~\cite{zhao2017pyramid}   & 21.18  & 53.01  &  $\sim$ 1056\\
Mip-NeRF~\cite{barron2021mip} + PSPNet~\cite{zhao2017pyramid}    & 21.54  & 51.15  &  $\sim$ 1056 \\
PNF~\cite{kundu2022panoptic}                  & \textbf{21.91}  & \underline{74.28} & $\sim$ 1256  \\
Ours                                                             & \underline{21.69}  & \textbf{75.07} & $\sim$ 244 \\ \hline
\end{tabular}
} %< \resizebox
   \vspace{-0.8em}
\caption{
% 
Results on novel view color and semantic synthesis tasks on KITTI-360~\cite{kitti360}. Nerflets achieve similar color synthesis quality and better semantic synthesis quality compared to PNF~\cite{kundu2022panoptic} without any 3D supervision. We also have the best efficiency in terms of worst case kFLOPs.
% 
} % \caption
\label{tab:kitti360}
\end{table}

==> [CVPR 2023] nerflets/tables/scannet3d_semins.tex <==
% \begin{table}
% \centering
% \resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
% \begin{tabular}{c|lcc}
% \hline
% &Method                                                           & Semantics mIoU  & Instance mAP\footnotesize{0.5} \\ \hline
% \multirow{5}{*}{3D}&MinkowskiNet~\cite{}      & 71.92  & -                 \\ 
% 3DMV~\cite{}     & 49.22  & -   \\  %\hline
% PointNet++~\cite{}   & 35.43  & -     \\
% Mask3D~\cite{}    & -  & 75.34      \\
% % SoftGroup~\cite{}    & -  & 72.83      \\
% 3D-BoNet~\cite{}    & -  & 46.23      \\  \hline
% Multiview Fusion~\cite{genova2021learning} & ???? & - \\
% Ours                               & 63.94  & 48.67  \\ \hline
% \end{tabular}
% } %< \resizebox
% \caption{
% Evaluation of nerflet panoptic performance on ScanNet 3D pointcloud labeling task. Nerflets beat some less recent fully 3D-supervised methods with less supervision at both semantic and instance tasks, while also beating the similarly supuervised multiview fusion approach.
% % 
% \reviseme{fix citations}
% % 
% } % \caption
% \label{tab:scannet3d}
% \end{table}
% \vspace{-1.3em}



\begin{table}
\centering
\resizebox{0.95\linewidth}{!}{ %< auto-adjusts font size to fill line
\begin{tabular}{c|ccc}
\hline
Supervision          & Method           & Semantics mIoU & Instance mAP\footnotesize{0.5} \\ \hline
\multirow{5}{*}{Pointcloud}           & MinkowskiNet~\cite{choy20194d}               & \textbf{71.92}          & -            \\
                              & 3DMV~\cite{dai20183dmv}                      & 49.22          & -            \\
                              & PointNet++~\cite{qi2017pointnet++}           & 44.54          & -            \\
                              & Mask3D~\cite{Schult22}                       & -              & \textbf{75.34}        \\
                              & 3D-BoNet~\cite{yang2019learning}             & -              & 46.23        \\ \hline
\multirow{2}{*}{Images}           & Multiview Fusion~\cite{genova2021learning}   & 55.23           & -            \\
                              & Ours                                         & \textbf{63.94}          & 48.67        \\ \hline
\end{tabular}
}
\vspace{-0.8em}
\caption{
Evaluation of nerflet panoptic performance on ScanNet 3D point cloud labeling task. Nerflets beat some less recent fully 3D-supervised methods with less supervision at both semantic and instance tasks, while also beating the similarly supervised multiview fusion approach.
}
\label{tab:scannet3d}
\end{table}

==> [CVPR 2023] nerflets/tables/scannet_nvs.tex <==
\begin{table}
\centering
\vspace{-0.3em}
\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
\begin{tabular}{lccc}
\hline
Method                                            & PSNR  & Semantics mIoU  & Instance mAP\footnotesize{0.5}\\ \hline
%NeRF~\cite{mildenhall2021nerf}                    & ?     & -  & -     \\
%Mip-NeRF~\cite{mildenhall2021nerf}                & ?     & -  & -     \\
PSPNet~\cite{zhao2017pyramid} on GT Image                     & -     & 68.43  & -     \\
Mask R-CNN~\cite{he2017mask}  on GT Image                      & -     & -     & 23.53  \\
\hline
PSPNet~\cite{zhao2017pyramid} on NeRF Im.                     & -     & 46.21  & -     \\
Mask R-CNN~\cite{he2017mask}  on NeRF Im.                      & -     & -     & 14.32  \\
Semantic-NeRF~\cite{Zhi21iccv_SemanticNeRF}       & 28.43  & 71.34  & -     \\
% Ours (w/o Instance)                               & \textbf{29.14}  & \textbf{73.78}  & -     \\  \hline
DM-NeRF~\cite{wang2022dmnerf}                     & 28.21  & 70.71  & 25.12  \\
Ours                                              & \textbf{29.12}  & \textbf{73.63}  & \textbf{31.32}  \\  \hline
\end{tabular}
} %< \resizebox
\vspace{-0.8em}
\caption{
% 
ScanNet novel view synthesis quantitative results. Rendered color images and segmentation maps from nerflets have the best quality among all evaluated methods.
} % \caption
\label{tab:scannet}
\end{table}

==> sections/background.tex <==

\reviseme{Let's try to squeeze this into method, or maybe assume it's already known?}
\textbf{Neural Radiance Field (NeRF)} Only recently, NeRF~\cite{mildenhall2021nerf} has been proposed to achieve photo-realistic novel view synthesis from only posed 2D images. Follow-up methods extend the framework in terms of generalizability~\cite{}, scalability~\cite{}, efficiency~\cite{}, interprebility~\cite{} and more information~\cite{}. Given a set of posed images $I_1$,...,$I_l$ of a scene with their known camera parameters $\Phi_1$,...,$\Phi_l$. NeRF~\cite{mildenhall2021nerf} uses an MLP to learn the 3D geometry and appearance information of the scene. More specifically, it learns a continuous scene function $F$ whose input is a location $\bfx=(x,y,z)$ and a viewing direction $\bfd = (\theta, \phi)$, and whose output is an emitted color $\bfc=(r,g,b)$ and volume density $\sigma$, representing local geometry and appearance information respectively. NeRF then use a discretized version of classical volume rendering~\cite{} to generate the estimated pixel color $\hat{C}(\bfr)$ for camera ray $\bfr(t)=\bfo+t\bfd$:
\begin{align}
\label{eq:nerf_raymarching}
\hat{C}(\bfr) &=\sum_{i=1}^N T_i \alpha_i \bfc_i, \\
\text{where\ \ }
 \alpha_i &= 1-\exp \left(-\sigma_i \delta_i\right), \\
%& T_i=\exp \left(-\sum_{j=1}^{i-1} \sigma_j \delta_j\right),
 T_i &=\prod_{j=1}^{i-1} (1-\alpha_j),
\end{align}
where $t_i$ are stratified samples along the ray in $N$ evenly-spaced bins, and $\delta_i=t_{i+1}-t_i$ the distance between adjacent samples.
% \xiaoshuai{I want to cover these equations for later reference. Separating this yields a very short preliminaries section.}


==> sections/limitations.tex <==
NOTE: THIS IS MOVED TO END OF CONCLUSION TO SAVE SPACE

Nerflets have several limitations. One limitation is that they do not model dynamic scene content. This is one potential direction for future work, because in principle the irregular nature of the representation could be leveraged to track moving or articulated objects.  Another is that we currently assume a fixed number of nerflets for the scene, regardless of the scene complexity, similar to a standard MLP. However, it may be advantageous to prune, add, or otherwise dynamically adjust the number based on where they are needed in the scene (e.g., where the loss is highest).

==> tables/abl_semvsapp.tex <==
\begin{table}
\centering
\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
\begin{tabular}{lccc}
\hline
                             & PSNR             & SSIM              & LPIPS  \\ \hline
Ours (w/o sem supervision)   & 20.95            & 0.778             & 0.343  \\
Ours (full model)            & \textbf{22.43}   & \textbf{0.820}    & \textbf{0.212}  \\  \hline
\end{tabular}
} %< \resizebox
\caption{
% 
Ablation experiment on our KITTI-360 validation set for the effectiveness of our semantic supervision. Representation learned with semantic supervision also achieves better performance on novel view synthesis.
} % \caption
\label{tab:abl_semvsapp}
\end{table}
